Cost Splitting for Multi-Objective Conflict-Based Search

The Multi-Objective Multi-Agent Path Finding (MO-MAPF) problem is the problem of finding the Pareto-optimal frontier of collision-free paths for a team of agents while minimizing multiple cost metrics. Examples of such cost metrics include arrival times, travel distances, and energy consumption.In this paper, we focus on the Multi-Objective Conflict-Based Search (MO-CBS) algorithm, a state-of-the-art MO-MAPF algorithm. We show that the standard splitting strategy used by MO-CBS can lead to duplicate search nodes and hence can duplicate the search effort that MO-CBS needs to make. To address this issue, we propose two new splitting strategies for MO-CBS, namely cost splitting and disjoint cost splitting. Our theoretical results show that, when combined with either of these two new splitting strategies, MO-CBS maintains its completeness and optimality guarantees. Our experimental results show that disjoint cost splitting, our best splitting strategy, speeds up MO-CBS by up to two orders of magnitude and substantially improves its success rates in various settings.

==> backup_cost_splitting.tex <==
\section{Cost Splitting}

% In this section, we describe a new splitting strategy for MO-CBS, called cost splitting, which usually generates fewer CT nodes than the standard splitting and still retains the completeness and optimality guarantees of MO-CBS.

The following example shows that MO-CBS can generate identical CT nodes during the search, which duplicate the search effort.

\begin{example}
Consider CT nodes $n_3$ and $n_6$ in Figure~\ref{fig:example_ct}. Both CT nodes contains the same set of constraints and path for each agent, which makes these two CT nodes indistinguishable from each other.
CT nodes $n_4$ and $n_7$ are indistinguishable from each other, too, since they share the same set of constraints and same set of paths.
In our example, CT nodes $n_3$ and $n_6$ are both conflict-free. However, for an MO-MAPF instance with more agents, such duplicate CT nodes can contain conflicts between other agents, and, to resolve these conflicts, MO-CBS repeats the search effort in the search tree that is rooted in these duplicate CT nodes.
\end{example}

% The idea of cost splitting is to 




\add{
In this section, we describe cost splitting, which generates fewer CT nodes than the standard splitting and still retains the completeness and optimality guarantees of MO-CBS.
For each CT node $n$ and each agent $a_i$, MO-CBS with cost splitting maintains a \emph{cost lower bound} $n.\mathbf{lb}=[n.\mathbf{lb}_1\ldots n.\mathbf{lb}_m]$. 
\begin{definition}
A path $\pi_i$ of agent $a_i$ is compatible with CT node $n$ iff:
\begin{enumerate}
    \item $n.\mathbf{lb}_i \preceq \mathbf{c}(\pi_i)$
    \item $\pi_i$ satisfies all constraints of CT node $n$
\end{enumerate}
A solution $\Pi$ is compatible with CT node $n$ iff all its paths are compatible with CT node $n$.
\label{def:compatible_old}
\end{definition}
}

\add{
During the initialization, MO-CBS with cost splitting initializes the cost lower bound of each agent in each root CT nodes to the path cost of the agent.
For every root CT node, all of its paths are compatible with it.
The cost lower bound of CT nodes $n_1$ and $n_2$ in Figure~\ref{fig:example_ct} are initialized to $[(1.5, 3), (4,4)]$ and $[(3, 2), (4,4)]$, respectively.
}

\add{
Algorithm~\ref{alg:cost-split} describes $\textsc{Split}()$ function of cost splitting.
For each agent $a_i$ involved in the conflict and the corresponding constraint $cons_i$, cost splitting calls its low level planner to replan a cost-unique Pareto-optimal frontier $\Pi_i'$ considering constraints $n.constraints \cup \{ cons_i\}$ (Line~\ref{line:cost_split_lowlevel}).
It then computes a set of vectors
$$\mathbf{LB}_i = ND(\{comax(n.\mathbf{lb}_i, \mathbf{c}(\pi))| \mathbf{\pi} \in \Pi_i'\}).$$
For each cost vector $\mathbf{lb}\in \mathbf{LB}_i$, MO-CBS creates a child CT node whose cost lower bound for agent $a_i$ is set to $\mathbf{lb}$ (Line~\ref{line:set_lower_bound}).
The following property shows that any compatible solution of the CT node $n$ is considered by at least one child CT node, which is the basis for retaining the optimality and completeness of MO-CBS.
\begin{property}
Any solution $\Pi$ that is compatible with CT node $n$ and satisfies the new constraint $cons_i$ is compatible with at least one child CT node generated for the subproblem with new constraint $cons_i$ being added to CT node $n$.
\label{prop2}
\end{property}
\begin{proof}
We use $\pi_i$ to denote the path for agent $a_i$ in solution $\Pi$. 
Because cost splitting only replans paths and updates cost lower bounds for agent $a_i$, according to Definition~\ref{def:compatible_old}, we only need to prove there exist a vector $lb \in \mathbf{LB}_i$ such that $lb \preceq \mathbf{c}(\pi_i)$.

Since $\Pi_i'$ is a cost-unique Pareto-optimal frontier (line~\ref{line:cost_split_lowlevel}), there exists a path $\pi^* \in \Pi_i'$ such that $\mathbf{c}(\pi^*)\preceq \mathbf{c}(\pi_i)$.
Because $n.\mathbf{lb}_i \preceq \mathbf{c}(\pi_i)$, we have $comax(n.\mathbf{lb}_i, \mathbf{c}(\pi^*)) \preceq \mathbf{c}(\pi_i)$. Since $comax(n.\mathbf{lb}_i, \mathbf{c}(\pi^*))$ is either in $\mathbf{LB}_i$ or dominated by a vector in $\mathbf{LB}_i$, the property holds.
\end{proof}
% To do so, cost splitting first replans a new cost-unique Pareto-optimal frontier $\Pi_i$ for agent $a_i$, and, for each path $\pi_i$ in $\Pi_i$, creates a new CT node whose cost lower bound for $a_i$ is $comax(n.\mathbf{lb}_i, \mathbf{c}(\pi_i))$.
% Intuitively, any path of $a_i$ that is compatible with $n$ (and hence is weakly dominated by $n.\mathbf{lb}_i$) and satisfies the new constraint must be weakly dominated by some path $\pi_i$ in $\Pi_i$.
% Therefore, by Property~\ref{prop0}, it is weakly dominated by $comax(n.\mathbf{lb}_i, \mathbf{c}(\pi_i))$ and hence compatible with the corresponding child CT node.
For child CT node with new cost lower bound for agent $a_i$ as $\mathbf{lb}$, the path of agent $a_i$ is set to the corresponding path of $\mathbf{lb}$ in $\Pi_i$ (Line~\ref{line:set_lower_bound}).
When splitting a CT node, cost splitting always generates no more child CT nodes than that generated by standard splitting because the size of $\mathbf{LB}_i$ is at most the size of $\Pi'_i$.
}

\add{
Consider CT node $n_1$ in Figure~\ref{fig:example_ct}.
The new cost-unique Pareto-optimal frontier for agent $a_1$ consists of two paths, denoted as $\pi_1^{(1)} = [A, B, B, D]$ (with $\mathbf{c}(\pi_1^{(1)}) = (4,2)$) and $\pi_1^{(2)}= [A, C, C, D]$ (with $\mathbf{c}(\pi_1^{(2)}) = (2.5,3)$).
Cost splitting creates two child CT node, which corresponds to CT nodes $n_3$ and $n_4$ in Figure~\ref{fig:example_ct} and whose cost lower bounds for $a_1$ are $n_3.\mathbf{lb}_1 = comax(n_1.\mathbf{lb}_1, \mathbf{c}(\pi_1^{(1)}))=(4,3)$ and $n_4.\mathbf{lb}_1 = comax(n_1.\mathbf{lb}_1, \mathbf{c}(\pi_1^{(2)}))=(2.5,3)$, respectively.
Since $(4,3)$ is weakly dominated by $(2.5,3)$, every compatible path of $n_3$ is compatible with $n_4$. CT node $n_3$ is discarded and Requirement 1 is still satisfied.
% Eventually, cost splitting only generate one child CT node, that is, $n''$, for this sub-problem. 
This is better than standard splitting, which generates two child CT nodes. 
The path of $a_1$ in $n_4$ is set to $\pi_1^{(2)}$, which is a compatible path of $n_4$ and also weakly dominates every compatible path of $n_4$ since $\pi_1^{(2)} = n_4.\mathbf{lb}_1$.
Consider CT node $n_2$ and the sub-problem with constraint $\langle a_1, D, 2\rangle$ when splitting it.
Cost splitting creates two child CT node, which corresponds to CT nodes $n_6$ and $n_7$ in Figure~\ref{fig:example_ct} and whose cost lower bounds for $a_1$ are $n_6.\mathbf{lb}_1 =comax(n_2.\mathbf{lb}_1, \mathbf{c}(\pi_1^{(1)}))=(4,2)$ and $n_7.\mathbf{lb}_1 = comax(n_2.\mathbf{lb}_1, \mathbf{c}(\pi_1^{(2)}))=(3,3)$, respectively.
The path of $a_1$ in $n_6$ and $n_7$ are set to $\pi_1^{(1)}$ and $\pi_1^{(=2)}$, respectively.
Note that the path of $a_1$ (with cost $(2.5, 3)$) in CT node $n_7$ is not compatible with it. 
As we will show later, this does not affect the optimality and completeness of MO-CBS since the path cost dominates $n_7.\mathbf{lb}_1$ and hence dominates all paths of agent $a_1$ that are compatible with  CT node $n_7$.
}

% For simplicity, we denote CT node $n_i$'s path of $a_1$ as $\pi_i$ in Figure~\ref{fig:example}. 
% To settle the above problem, we start from initialization. 
% We know $\pi_1$ and $\pi_2$ are the only two Pareto frontiers for agent $a_1$ ignoring constraints. For any path $\pi$ for agent $a_1$, $\mathbf{c}(\pi)$ is dominated by either $\mathbf{c}(\pi_1)$ or $\mathbf{c}(\pi_2)$. Thus here we split the paths for $a_1$ into two parts (there maybe repetitions) by its dominance relationship with $\mathbf{c}(\pi_1)$ or $\mathbf{c}(\pi_2)$. Using such a property, we set a lower bound for $n_1$ and $n_2$ as $\mathbf{c}(\pi_1)$ and $\mathbf{c}(\pi_2)$ seperately. 
% This means that $n_1$ and its child CT nodes aim at those paths of agent $a_1$ whose costs are weakly dominated by the set lower bound and the same to $n_2$.

% After adding constraint $\langle a_1, D, 2\rangle$ to $n_1$, we get new Pareto frontiers for agent $a_1$, denoted as $\pi_3 = [A, B, B, D]$ and $\pi_4 = [A, C, C, D]$, and generate new CT nodes $n_3$ and $n_4$. Note that we don't use the previous lower bound to restrict our low-level search because lower bound will lead to much worse performance in low-level search. We continue applying the above property and update the lower bound. For $n_3$, it aims at paths whose costs are weakly dominated by both $\mathbf{c}(\pi_1)$ and $\mathbf{c}(\pi_3)$ which is equal to being dominated by $comax(\mathbf{c}(\pi_1), \mathbf{c}(\pi_3)) = comax((1.5, 3), (4, 2)) = (4, 3)$. This will be the lower bound for $n_3$. Similarly, lower bound for $n_4$ will be $comax((1.5, 3), (2.5, 3)) = (2.5, 3)$. Because $(2.5, 3) \prec (4, 3)$, paths considered by $n_3$ must be considered by $n_4$ already. This provides us with space to prune $n_3$. Figure~\ref{alg:cost-split} shows detailed lower bound for each generated CT node in Figure~\ref{fig:example}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.35\textwidth]{fig/cost_splitting_v2.png}  
    \caption{Node generation after using cost splitting. We use the cost on agent $1$ to represent each node. $n_1$ will only generate $n_4$, and $n_3$ will be pruned.
    \hz{change $n_1$ to $\mathbf{n_1.\mathbf{lb}_1}$ and $n_3$ and $n_4$ to actual numbers?}
    }
    \label{fig:cost_splitting}
\end{figure}

% In above approach, any path for agent $a_1$ is considered by at least one CT node after each low-level splitting. This is the basis for ensuring the completeness of our algorithm.

% Next, we formalize our approach. For each CT node $n$ and each agent $a_i$, MO-CBS with cost splitting maintains a \emph{cost lowerbound} $n.\mathbf{lb}=[n.\mathbf{lb}_1\ldots n.\mathbf{lb}_m]$, which means CT node $n$ are aiming at paths whose cost are dominated by $\mathbf{lb}_i$. We don't necessarily require the path of $n$ itself to satisfy this property.

% During the initialization, MO-CBS with cost splitting initializes the cost lower bound of each agent in each root CT nodes to the path cost of the agent.
Algorithm~\ref{alg:cost-split} \add{formally describes the} $\textsc{Split}()$ function \add{for cost splitting}.
For each agent $a_i$ involved in the conflict, cost splitting calls its low level planner to replan a cost-unique Pareto-optimal frontier $\Pi_i'$ of the paths of $a_i$(Line~\ref{line:cost_split_lowlevel}).
\add{It then} computes a set of cost vectors
$$\mathbf{LB}_i = ND(\{comax(n.\mathbf{lb}_i, \mathbf{c}(\pi))| \mathbf{\pi} \in \Pi_i'\}).$$
For each cost vector $\mathbf{lb}\in \mathbf{LB}_i$, MO-CBS creates a child CT node and sets the lower bound for agent $a_i$ to $\mathbf{lb}$ and set a corresponding path (line~\ref{line:set_lower_bound}).
When splitting a CT node, cost splitting always generates no more child CT nodes than that generated by standard splitting because the size of $\mathbf{LB}_i$ is at most the size of $\Pi'_i$.

% Here we define compatibility to introduce two properties of MO-CBS with cost splitting.

% \begin{definition}
% Given a CT node $n$, a path $\pi_i$ of agent $a_i$ is compatible with CT node $n$ iff the following properties hold:
% \begin{enumerate}
%     \item $n.\mathbf{lb}_i \preceq \mathbf{c}(\pi)$
%     \item $\pi_i$ satisfies all constraints of CT node $n$
% \end{enumerate}
% A solution $\Pi$ is compatible with a CT node $n$ iff all its paths are compatible with CT node $n$.
% \label{def:compatible_old}
% \end{definition}

The following Properties~\ref{prop1} and~\ref{prop2} show that, conceptually, $\mathbf{LB}_i$ corresponds to a set of cost regions that are ``refined'' from the cost region represented by $n.\mathbf{lb}_i$, and every compatible path of $a_i$ in the successor CT nodes of $n$ lies in at least one of these cost regions.
As we will show later, Property~\ref{prop2} is important for maintaining the completeness and optimality guarantees of MO-CBS.


\begin{property}
Any cost vector $\mathbf{lb}\in \mathbf{LB}_i$ is weakly dominated by $n.\mathbf{lb}_i$.
\label{prop1}
\end{property}
\begin{proof}
The property holds because $\mathbf{lb}$ is the component-wise maximum of $n.\mathbf{lb}_i$ and another vector and is hence weakly dominated by $n.\mathbf{lb}_i$.
\end{proof}
\begin{property}
For any solution $\Pi$ that satisfies constraints $n.constraints \cup \{cons\}$ (Line~\ref{line:constraint-union}) and is compatible with CT node $n$, $\Pi$ is still compatible with at least one child node generated by the subproblem with new constraint $cons$ being added to CT node $n$.
\label{prop2}
\end{property}
\begin{proof}
We use $a_i$ to denote the agent to which the constraint $cons$ applied, and $\pi_i$ to denote the path for agent $a_i$ in solution $\Pi$. Because we will only replan paths for $a_i$, according to Definition~\ref{def:compatible_old}, we only need to prove there exist a vector $lb \in \mathbf{LB}_i$ such that $lb \preceq \mathbf{c}(\pi_i)$.

Since $\Pi_i'$ is a cost-unique Pareto-optimal frontier (line~\ref{line:cost_split_lowlevel}), there exists a path $\pi^* \in \Pi_i'$ such that $\mathbf{c}(\pi^*)\preceq \mathbf{c}(\pi_i)$.
Because $n.\mathbf{lb}_i \preceq \mathbf{c}(\pi_i)$, we have $comax(n.\mathbf{lb}_i, \mathbf{c}(\pi^*)) \preceq \mathbf{c}(\pi_i)$. Since $comax(n.\mathbf{lb}_i, \mathbf{c}(\pi^*))$ is either in $\mathbf{LB}_i$ or dominated by a vector in $\mathbf{LB}_i$, the property holds.
\end{proof}

\begin{algorithm}[t]
    \footnotesize
    \input{algoconf.tex}
   
    \Fn{\textsc{Split}$(n, \mathit{conf})$}{
        $children \gets \emptyset$\;
         \ForEach{ $a_i$ involved in $\mathit{conf}$ and the corresponding contraint $cons_i$}{
            $C'_i \gets n.constraints \cup \{cons_i\}$ \label{line:constraint-union}\;
            $\Pi'_i \gets \textsc{LowLevelSearch}(a_i, C'_i)$ \label{line:cost_split_lowlevel} \;
            $\mathbf{LB}_i \gets ND(\{comax(n.\mathbf{lb}_i, \mathbf{c}(\pi))| \mathbf{\pi} \in \Pi_i'\})$ \;
            \ForEach{ $\mathbf{lb}\in \mathbf{LB}_i$}{
                $n' \gets n$\;
                $n'.constraints\gets C'_i$\;
                $n'.\mathbf{lb}_i \gets \mathbf{lb}$\; \label{line:set_lower_bound}
             $n'.plan[i]\gets$ a path $ \pi\in \Pi'_i$ such that $ comax(n.\mathbf{lb}_i, \mathbf{c}(\pi)) = \mathbf{lb}$\;
                add $n'$ to $children$\;
            }
        }
    \Return $children$\;
    }
\caption{Cost splitting}
\label{alg:cost-split}
\end{algorithm}

% \begin{example}
% Figure~\ref{fig:cost_splitting} shows the cost lower-bounds of agent $a_1$ in CT nodes $n_1$ and $n_2$ of Figure~\ref{fig:example} and the path costs of the cost-unique Pareto-optimal frontier of agent $a_1$ after constraint $\langle a_1, D, 2\rangle$ is added.
% During the initialization, $n_1.\mathbf{lb}_1$ and $n_2.\mathbf{lb}_1$ are set to path costs $(1.5, 3)$ and $(3, 2)$, respectively. 
% After adding constraint $\langle a_1, D, 2\rangle$, a cost-unique Pareto-optimal frontier of $a_1$ consists of paths $[A,B,B,D]$ and $[A,C,C,D]$, whose costs are $(2.5,3)$ and $(4,2)$, respectively.
% MO-CBS with cost splitting does not generate $n_3$ when splitting $n_1$ because $comax(n_1.\mathbf{lb}_1, (2.5,3)) = (2.5,3) \prec comax(n_1.\mathbf{lb}_1, (4,2)) = (4,3)$. 
% MO-CBS with cost splitting still generates $n_6$ and $n_7$ when splitting $n_2$ because vectors $comax(n_2.\mathbf{lb}_1, (2.5,3)) = (3,3)$ and $comax(n_2.\mathbf{lb}_1, (4,2)) = (4,2)$ do not dominate each other.
% Note that $n_6.\mathbf{lb}_1=(3,3)$ is unequal to but weakly dominated by the cost of the path of agent $a_1$ ($2.5, 3$) in $n_6$.
% \label{example:cost-split}
% \end{example}

% One may consider an alternative approach for cost splitting in which the low-level search algorithm finds a Pareto-optimal frontier $\Pi$ of paths that satisfies all constraints and whose costs are also weakly dominated by the cost lower bound.
% MO-CBS then creates a CT node for each path $\pi$ in $\Pi$ and, for each CT node and each agent, the cost lower bound is always equal to $\mathbf{\pi}$.
% Although this approach avoids cases like $n_6$ in Example~\ref{example:cost-split}, it requires a more complicated low-level search algorithm as existing multi-objective search algorithms do not handle lower bounds.

